Robot-to-Robot Transfer of Public VLA Checkpoints: Policy-Specific Failure Modes and Training-Free Corrections

Changing a robot's gripper can reduce manipulation success even when the task stays the same. We tested public checkpoints from five vision-language-action (VLA) policies in LIBERO simulation. Swapping the gripper's appearance and its physics separately revealed which change caused the larger loss for each policy. Across 12 original policy-gripper pairs, that comparison identified the better of two corrections: changing the wrist image or adjusting the gripper setup. One of four labels reversed on replication, so direct trials remain important when choosing a correction. For a rotated base frame, six probe motions let us calibrate commands for four relative-action policies without retraining. At $15^\circ$ yaw, successes rose from 18-74 to 87-114 per 120 episodes. Changes in wrist-image features ranked visual risk before execution, but missed failures caused by gripper physics. Two undocumented OpenVLA evaluation settings together changed success by 20 percentage points.

==> generated/tab_select.tex <==
\begin{tabular}{@{}llcccccc@{}}
\toprule
Gripper & Policy & Diagnosis A/P & Selected & None & DT-Comp & Bracket & Both \\
\midrule
OnRobot 2FG7 & X-VLA & 0/43 & DT-Comp & 0 & \textbf{39} & 14 & 33 \\
 & $\pi_{0.5}$ & 2/35 & DT-Comp & 1 & \textbf{39} & 30 & 31 \\
 & GR00T & 72/29 & bracket & 17 & 22 & \textbf{65} & 66 \\
 & $\tau_0$ & 49/9 & bracket & 17 & 8 & \textbf{42} & 38 \\
\midrule
Robotiq Hand-E & X-VLA & 0/59 & DT-Comp & 0 & \textbf{50} & 3 & 16 \\
 & $\pi_{0.5}$ & 0/48 & DT-Comp & 0 & \textbf{31} & 5 & 22 \\
 & GR00T & 68/56 & bracket & 44 & 55 & \textbf{75} & 57 \\
 & $\tau_0$ & 27/25 & bracket & 9 & 18 & \textbf{45} & 40 \\
\midrule
DH PGC-50-35 & X-VLA & 0/81 & DT-Comp & 0 & \textbf{75} & 0 & 72 \\
 & $\pi_{0.5}$ & 5/52 & DT-Comp & 3 & \textbf{46} & 11 & 50 \\
 & GR00T & 55/73 & DT-Comp & 46 & \textbf{67} & 46 & 66 \\
 & $\tau_0$ & 63/49 & bracket & 9 & 27 & \textbf{42} & 63 \\
\bottomrule
\end{tabular}
\\[2pt]
\parbox{0.8\textwidth}{\scriptsize Panda baseline of the same run (successes out of 100): 2FG7 run: X-VLA 91, $\pi_{0.5}$ 85, GR00T 95, $\tau_0$ 96; Hand-E/PGC-50-35 run: X-VLA 91, $\pi_{0.5}$ 85, GR00T 95, $\tau_0$ 96.}

